Generalized Mirror Prox for Monotone Variational Inequalities: Universality and Inexact Oracle

We introduce an inexact oracle model for variational inequalities (VI) with monotone operator, propose a numerical method which solves such VI's and analyze its convergence rate. As a particular case, we consider VI's with H\"older-continuous operator and show that our algorithm is universal. This means that without knowing the H\"older parameter $\nu$ and H\"older constant $L_{\nu}$ it has the best possible complexity for this class of VI's, namely our algorithm has complexity $O\left( \inf_{\nu\in[0,1]}\left(\frac{L_{\nu}}{\varepsilon} \right)^{\frac{2}{1+\nu}}R^2 \right)$, where $R$ is the size of the feasible set and $\varepsilon$ is the desired accuracy of the solution. We also consider the case of VI's with strongly monotone operator and generalize our method for VI's with inexact oracle and our universal method for this class of problems. Finally, we show, how our method can be applied to convex-concave saddle point problems with H\"older-continuous partial subgradients.

==> UMP to arxiv 2022/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{verbatim}    %% for using command \begin{comment} \end{comment}
\usepackage{multirow}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\newcommand\funding[1]{\protect\\ \hspace*{15.37pt}{\bfseries Funding:} #1}
\newcommand{\email}[1]{\protect\href{mailto:#1}{#1}}


% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Generalized Mirror Prox Algorithm for Monotone Variational Inequalities: Universality and Inexact Oracle
%Solving Variational Inequalities with Monotone Operator, Inexact Oracle, and Unknown H\"older Parameters
\thanks{Submitted to the editors DATE.
%\funding{The research by P. Dvurechensky, A. Gasnikov and F. Stonyakin in Section 2 was funded by Russian Foundation for Basic Research (project 18-31-20005 mol-a-ved). The research by P. Dvurechensky and A. Gasnikov in Sections 1, 3 and 4 was funded by Russian Science Foundation (project 17-11-01027). The research by F. Stonyakin in Section 5 and Appendixes B1 and B3 was supported by Russian Science Foundation (project 18-71-00048).}
}}

\makeatletter
\let\@fnsymbol\@arabic
\makeatother

% Authors: full names plus addresses.
\author{
Fedor Stonyakin
\thanks{V.I. Vernadsky Crimean Federal University, Simferopol; Moscow Institute of Physics and Technology, Moscow
  (\email{fedyor@mail.ru}).}
\and Alexander Gasnikov
\thanks{Moscow Institute of Physics and Technology, Moscow; Institute for Information Transmission Problems RAS, Moscow
	(\email{gasnikov@yandex.ru}).}
\and Pavel Dvurechensky
\thanks{Weierstrass Institute for Applied Analysis and Stochastics, Berlin
	(\email{pavel.dvurechensky@wias-berlin.de}).}	
\and Alexander Titov
\thanks{Moscow Institute of Physics and Technology, Moscow
	(\email{a.a.titov@phystech.edu}).}
\and Mohammad S. Alkousa
\thanks{Moscow Institute of Physics and Technology, Moscow
	(\email{mohammad.alkousa@phystech.edu}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

